Freezing 1-Tag Systems with States

We study 1-tag systems with states obeying the freezing property that only allows constant bounded number of rewrites of symbols. We look at examples of languages accepted by such systems, the accepting power of the model, as well as certain closure properties and decision problems. Finally we discuss a restriction of the system where the working alphabet must match the input alphabet.

==> eptcsdata.tex <==
\providecommand{\firstpage}{82}
\providecommand{\publicationstatus}{Zs. Gazdag, Sz. Iv\'an, G. Kov\'asznai (Eds.): 16th International\\Conference on Automata and Formal Languages (AFL 2023)\\
EPTCS 386, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.386.8}{10.4204/EPTCS.386.8}}
\pdfoutput=1


==> figures/astarbstar.tex <==
\begin{tikzpicture}[scale=0.13]
\color{red}
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (31.1,-26.6) circle (3);
\draw (31.1,-26.6) node {$2$};
\draw [black] (44.4,-26.6) circle (3);
\draw (44.4,-26.6) node {$3$};
\draw [black] (17.9,-26.6) circle (3);
\draw (17.9,-26.6) node {$1$};
\draw [black] (57.7,-26.6) circle (3);
\draw (57.7,-26.6) node {$4$};
\draw [black] (57.7,-26.6) circle (2.4);
\draw [black] (34.1,-26.6) -- (41.4,-26.6);
\fill [black] (41.4,-26.6) -- (40.6,-26.1) -- (40.6,-27.1);
\draw (37.75,-26.1) node [above] {$b/y$};
\draw [black] (29.777,-23.92) arc (234:-54:2.25);
\draw (31.1,-19.35) node [above] {$a/x$};
\fill [black] (32.42,-23.92) -- (33.3,-23.57) -- (32.49,-22.98);
\draw [black] (43.077,-23.92) arc (234:-54:2.25);
\draw (44.4,-19.35) node [above] {$b/y$};
\fill [black] (45.72,-23.92) -- (46.6,-23.57) -- (45.79,-22.98);
\draw [black] (20.9,-26.6) -- (28.1,-26.6);
\fill [black] (28.1,-26.6) -- (27.3,-26.1) -- (27.3,-27.1);
\draw (24.5,-26.1) node [above] {$a/f$};
\draw [black] (11.2,-26.6) -- (14.9,-26.6);
\fill [black] (14.9,-26.6) -- (14.1,-26.1) -- (14.1,-27.1);
\draw [black] (47.4,-26.6) -- (54.7,-26.6);
\fill [black] (54.7,-26.6) -- (53.9,-26.1) -- (53.9,-27.1);
\draw (51.05,-26.1) node [above] {$f/f$};
\end{tikzpicture}

